Protecting Privacy in Classifiers by Token Manipulation

Using language models as a remote service entails sending private information to an untrusted provider. In addition, potential eavesdroppers can intercept the messages, thereby exposing the information. In this work, we explore the prospects of avoiding such data exposure at the level of text manipulation. We focus on text classification models, examining various token mapping and contextualized manipulation functions in order to see whether classifier accuracy may be maintained while keeping the original text unrecoverable. We find that although some token mapping functions are easy and straightforward to implement, they heavily influence performance on the downstream task, and via a sophisticated attacker can be reconstructed. In comparison, the contextualized manipulation provides an improvement in performance.

==> 03_attack.tex <==
In order to test the resilience of these techniques against token inversion attacks, a possible attacker can exploit the fact that the process utilizes contextualized tokens and the selection of the nearest token.
Specifically, the attacker can compute the euclidean distance or cosine similarity between the perturbed token and the word embedding matrix, and select the nearest token as the reconstruction result.







==> latex_tips.tex <==

\uvp{\small
Some of my \LaTeX{} rules:
Full parenthetical citations (\texttt{\textbackslash{}cite} or \texttt{\textbackslash{}citep}) are preceded by a NBSP (tilde).
Each sentence gets its own source line (so it can be easily found, moved around, commented out).
We use \say{\texttt{\textbackslash{}say}} for quotes.
We don't use \texttt{\textbackslash{}subsubsections}---stuff below \texttt{\textbackslash{}subsection} gets \texttt{\textbackslash{}paragraph}.
We don't use \texttt{\textbackslash{}vspace} and its friends, definitely not in drafts.
When we have enough prose in a section (or sooner, whatever's convenient), we extract it to its own file.
\url{http://detexify.kirelabs.org/classify.html} is a life-saver.
We use macros for names and terms that might change, like system names, and for inconveniently long but often-used phrases.
Numbers in the body of the text don't get put in mathmode.
Tables: no vertical lines, ever.
Minimal horizontal lines, using the \texttt{\textbackslash{}booktabs} extension (toprule and bottomrule in borders, midrule below legend and between coarse-grain row groups).
Anything that was published in a peer-reviewed venue is cited by its published venue, not arXiv.
If it was in an ACL-indexed venue, all you have to do is look it up on the anthology website (I have a Chrome shortcut for anthology search) and single-click-copy the bibkey, since we have the bib file already. Example:~\cite{klymenko-etal-2022-differential}.
For more: \href{https://medium.com/@vered1986/tips-for-writing-nlp-papers-9c729a2f9e1f}{here.}}


==> tables/9_full_table.tex <==
\begin{table*}
\begin{tabular}{l|c|cc|cc}
\toprule
  \textbf{Dataset} & \textbf{Mapper}  & \textbf{Test} &\textbf{Train+Test} & \textbf{Token@1} & \textbf{Token@5} \\ \midrule
& Punc. \convdef{} & 0\% & 0\% \\
SST2 & \convdef{} (9, 0.8) & 27\% & 49\% \\
& Noise ($\eta=100)$  & 32\% & 70\% \\
& Noise ($\eta=150)$  & 34\% & 75\% \\
& \convdef{}($\sigma$=0.2) & 60\% & A\% \\
& \convdef{}($\sigma$=0.6) & 61\% & A\% \\
SST2 & \convdef{}($\sigma$=0.8) & 41\% & A\% \\
& \convdef{}($\sigma$=1.0) & 17\% & A\% \\
& \convdef{}(3, 0.2) & 86.0\%	& 91.9\% \\
& \convdef{}(5, 0.2) & 85.2\%	& 91.5\% \\
SST2 & \convdef{}(7, 0.2) & 85.4\% & 91.2\% \\
& \textbf{\convdef{}(9, 0.2) }& \textbf{87.2\%}	&\textbf{ 91.9\%} \\
& \convdef{}(11, 0.2) & 86.0\% & 91.2\% \\
\midrule
& \textbf{Fine tune} & \textbf{95\%} & \textbf{95\%} \\
 & Punc. \convdef{} & 85\% & 87\% \\
IMDB & \convdef{} (9, 0.8) & 83.5\% & 89.3\% \\
& Noise ($\eta=100)$  & 80\% & 87.8\% \\
& Noise ($\eta=150)$  & 83\% & 90\% \\

& \convdef{}(Window=3) & a\% & A\% \\
& \convdef{}(Window=5) & a\% & A\% \\
IMDB & \convdef{}(Window=7) & a\% & A\% \\
& \convdef{}(Window=9) & a\% & A\% \\
& \convdef{}(Window=11) & a\% & a\% \\
\bottomrule
\end{tabular}
\caption{The \convdef{} mapping capabilities in preserving privacy against an \say{KNN} attacker with different values of $\sigma$ with a window size of 9.}
\label{table:stencil_sigma_privacy}
\end{table*}

==> tables/9_table_punctuated_def.tex <==
\begin{table}
\begin{tabular}{lccc}
\toprule
  \textbf{Dataset} & \textbf{Mapper}  & \textbf{Token@1} & \textbf{Token@5} \\ \midrule
& Punc. \convdef{} & 0\% & 0\% \\
SST2 & \convdef{} (9, 0.8) & 27\% & 49\% \\
& Noise ($\eta=100)$  & 32\% & 70\% \\
& Noise ($\eta=150)$  & 34\% & 75\% \\
\midrule
& \textbf{Fine tune} & \textbf{95\%} & \textbf{95\%} \\
 & Punc. \convdef{} & 85\% & 87\% \\
IMDB & \convdef{} (9, 0.8) & 83.5\% & 89.3\% \\
& Noise ($\eta=100)$  & 80\% & 87.8\% \\
& Noise ($\eta=150)$  & 83\% & 90\% \\
\bottomrule
\end{tabular}
\caption{The \convdef{} mapping capabilities in preserving privacy against an \say{KNN} attacker with different values of $\sigma$ with a window size of 9.}
\label{table:stencil_sigma_privacy}
\end{table}

==> tables/9_table_stencil_acc.tex <==
\begin{table}
\begin{tabular}{lccc}
\toprule
Dataset & Mapper & Test & Train+Test \\
\midrule
& \textbf{Fine tune} & \textbf{94.5\%} & \textbf{94.5\%} \\
SST2 & \convdefshort{} & 62\% & 80\% \\
& Noise(100)$  & 81\% & 87\% \\
& Noise(200)$  & 83\% & 90\% \\
\midrule
& \textbf{Fine tune} & \textbf{95\%} & \textbf{95\%} \\
& 2-Random & 75\% & 90\% \\
IMDB & 3-Random & 68\% & 85\% \\
& High-freq & 93\% & 94\% \\
& Low-freq & 60\% & 80\% \\
\bottomrule
\end{tabular}
\caption{The three random mappings accuracy on SST2 and IMDB.}
\label{table:stencil_acc}
\end{table}

==> tables/9_table_stencil_sigma_privacy.tex <==
\begin{table}
\begin{tabular}{lccc}
\toprule
  \textbf{Dataset} & \textbf{Mapper}  & \textbf{Token@5} & \textbf{Exact-M}\\ \midrule
\multirow{4}{1em}{SST2} & \convdef{}($\sigma$=0.2) & 60\% & A\% \\
& \convdef{}($\sigma$=0.6) & 61\% & A\% \\
 & \convdef{}($\sigma$=0.8) & 41\% & A\% \\
& \convdef{}($\sigma$=1.0) & 17\% & A\% \\
\midrule
\multirow{4}{1em}{IMDb} & \convdef{}($\sigma$=0.2) & 60\% & A\% \\
& \convdef{}($\sigma$=0.6) & 61\% & A\% \\
& \convdef{}($\sigma$=0.8) & 41\% & A\% \\
& \convdef{}($\sigma$=1.0) & 17\% & A\% \\
\bottomrule
\end{tabular}
\caption{The \convdef{} mapping capabilities in preserving privacy against an \say{KNN} attacker with different values of $\sigma$ with a window size of 9.}
\label{table:stencil_sigma_privacy}
\end{table}

==> tables/9_table_stencil_window_privacy.tex <==
\begin{table}
\begin{tabular}{lccc}
\toprule
  \textbf{Dataset} & \textbf{Mapper}  & \textbf{Token@5} & \textbf{Exact-M}\\ \midrule
\midrule
& \convdef{}(Window=3) & A\%	& a\% \\
& \convdef{}(Window=5) & A\%	& a\% \\
SST2 & \convdef{}(Window=7) & a\% & a\% \\
& \convdef{}(Window=9) & a\%	& a\% \\
& \convdef{}(Window=11) & a\% & a\% \\
\midrule
& \convdef{}(Window=3) & a\% & A\% \\
& \convdef{}(Window=5) & a\% & A\% \\
 & \convdef{}(Window=7) & a\% & A\% \\
& \convdef{}(Window=9) & a\% & A\% \\
& \convdef{}(Window=11) & a\% & a\% \\
\bottomrule
\end{tabular}
\caption{The \convdef{} mapping capabilities in preserving privacy against an \say{KNN} attacker with different values of window sizes with a $\sigma=0.2$. This doesn't really have any infuelence, the results are not updates because i think its unnecesary}
\label{table:stencil_privacy_window}
\end{table}






